Interpretable Non-linear Survival Analysis with Evolutionary Symbolic Regression

Survival Regression (SuR) is a key technique for modeling time to event in important applications such as clinical trials and semiconductor manufacturing. Currently, SuR algorithms belong to one of three classes: non-linear black-box -- allowing adaptability to many datasets but offering limited interpretability (e.g., tree ensembles); linear glass-box -- being easier to interpret but limited to modeling only linear interactions (e.g., Cox proportional hazards); and non-linear glass-box -- allowing adaptability and interpretability, but empirically found to have several limitations (e.g., explainable boosting machines, survival trees). In this work, we investigate whether Symbolic Regression (SR), i.e., the automated search of mathematical expressions from data, can lead to non-linear glass-box survival models that are interpretable and accurate. We propose an evolutionary, multi-objective, and multi-expression implementation of SR adapted to SuR. Our empirical results on five real-world datasets show that SR consistently outperforms traditional glass-box methods for SuR in terms of accuracy per number of dimensions in the model, while exhibiting comparable accuracy with black-box methods. Furthermore, we offer qualitative examples to assess the interpretability potential of SR models for SuR. Code at: https://github.com/lurovi/SurvivalMultiTree-pyNSGP.

==> _legendak.tex <==
\definecolor{ktwo}{HTML}{C5F30C}
\definecolor{kthree}{HTML}{31AB0C}
\definecolor{kfour}{HTML}{283ADF}

\begin{figure*}[!htbp]
    \centering
    \begin{tikzpicture}
   
       
        \draw [line width=1.4mm, color=ktwo] (0,0) -- (0.4,0) node [right] {\textcolor{black}{$k = 3$}};
        \draw [line width=1.4mm, color=kthree] (1.7,0) -- (2.1,0) node [right] {\textcolor{black}{$k = 4$}};
        \draw [line width=1.4mm, color=kfour] (3.4,0) -- (3.8,0) node [right] {\textcolor{black}{$k = 5$}}; 
    
    \end{tikzpicture}
    %\tikzexternaldisable
    %\pgfplotslegendfromname{lineplot-100-1000-eucldist}
    %\tikzexternalenable
    \caption{prova}
    \label{fig:provalegenda}
\end{figure*}

==> _legendamethods.tex <==
\definecolor{SR}{HTML}{33B9F2}
\definecolor{CX}{HTML}{CBE231}
\definecolor{ST}{HTML}{E55E0F}
\definecolor{GB}{HTML}{0B1DBA}
\definecolor{RF}{HTML}{6B2106}



\begin{figure*}[!htbp]
    \centering
    \begin{tikzpicture}
   
       
        \draw [line width=1.4mm, color=SR] (0,0) -- (0.4,0) node [right] {\textcolor{black}{SR}};
        \draw [line width=1.4mm, color=CX] (1.4,0) -- (1.8,0) node [right] {\textcolor{black}{CX}};
        \draw [line width=1.4mm, color=ST] (2.8,0) -- (3.2,0) node [right] {\textcolor{black}{ST}};
        \draw [line width=1.4mm, color=GB] (4.2,0) -- (4.6,0) node [right] {\textcolor{black}{GB}};
        \draw [line width=1.4mm, color=RF] (5.6,0) -- (6.0,0) node [right] {\textcolor{black}{RF}};
    
    \end{tikzpicture}
    %\tikzexternaldisable
    %\pgfplotslegendfromname{lineplot-100-1000-eucldist}
    %\tikzexternalenable
    \caption{prova}
    \label{fig:provalegenda}
\end{figure*}

==> _legendatraintest.tex <==
\definecolor{train}{HTML}{E51D1D}
\definecolor{test}{HTML}{3B17F2}

\begin{figure*}[!htbp]
    \centering
    \begin{tikzpicture}
   
       
        \draw [line width=1.4mm, color=train] (0,0) -- (0.4,0) node [right] {\textcolor{black}{Train}};
        \draw [line width=1.4mm, color=test] (1.7,0) -- (2.1,0) node [right] {\textcolor{black}{Test}};
    
    \end{tikzpicture}
    %\tikzexternaldisable
    %\pgfplotslegendfromname{lineplot-100-1000-eucldist}
    %\tikzexternalenable
    \caption{prova}
    \label{fig:provalegenda}
\end{figure*}

==> citableblackbox.tex <==
% \begin{table*}
%     \centering
%     %\raggedleft
%     \renewcommand{\arraystretch}{0.8}
%     \caption{Median values (across the repetitions) of \CI from the Pareto front computed on the test set after the end of the optimization for the black-box methods.
%     Each black-box method employs all the features, and it is compared with SR with varying features.}
%     \label{tab:citableblackbox}
%     \begin{tabular}{
%     c
%     c
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     S[table-format=1.3]
%     }
%          \toprule
%  &  & \multicolumn{5}{c}{Normalization} & \multicolumn{5}{c}{No Normalization} \\
%  \cmidrule(lr){3-7} \cmidrule(lr){8-12}
%  $k$ & & {\PBC} & {\SPP} & {\FRM} & {\BCM} & {\BCR} & {\PBC} & {\SPP} & {\FRM} & {\BCM} & {\BCR} \\
%          \midrule


% \multirow{3}{*}{3} & GB & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.754{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & 0.668 & 0.617 & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & 0.667 & 0.619 \\ 
%   & RF & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.671 & \bfseries 0.621 & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.671 & \bfseries 0.621 \\ 
%   & SR & 0.758 & 0.652 & 0.736 & 0.668 & 0.615 & 0.756 & 0.648 & 0.736 & 0.669 & 0.615 \\ 
%  \midrule 
% \multirow{3}{*}{5} & GB & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.754{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & 0.668 & 0.617{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & 0.667 & 0.619 \\ 
%   & RF & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.671 & \bfseries 0.621 \\ 
%   & SR & 0.763 & 0.652 & 0.745 & 0.669 & 0.612 & 0.765 & 0.655 & 0.745 & 0.667 & 0.614 \\ 
%  \midrule 
% \multirow{3}{*}{7} & GB & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.754{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & 0.668 & 0.617{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & 0.667 & 0.619{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} \\ 
%   & RF & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75 & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75 & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} \\ 
%   & SR & 0.761 & 0.651 & 0.751 & 0.67 & 0.608 & 0.757 & 0.658 & 0.75 & 0.671 & 0.61 \\ 
%  \midrule 
% \multirow{3}{*}{\text{max}} & GB & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & 0.754{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.668 & 0.617{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.667 & 0.619{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} \\ 
%   & RF & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75 & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75 & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} \\ 
%   & SR & 0.77 & 0.649 & \bfseries 0.756{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.664 & 0.608 & 0.765 & 0.655 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.668 & 0.611 \\ 
  
 
 


  
%          \bottomrule
%     \end{tabular}
% \end{table*}


\begin{table*}[h]
    \centering
    %\raggedleft
    \renewcommand{\arraystretch}{0.8}
    \caption{Median values (across the repetitions) of \CI from the Pareto front computed on the test set after the end of the optimization for the black-box methods.
    Each black-box method employs all the features, and it is compared with SR model from the Pareto front with the maximum number of features.}
    \label{tab:citableblackbox}
    \begin{tabular}{
    c
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    S[table-format=1.3]
    }
         \toprule
   & \multicolumn{5}{c}{Normalization} & \multicolumn{5}{c}{No Normalization} \\
 \cmidrule(lr){2-6} \cmidrule(lr){7-11}
   & {\PBC} & {\SPP} & {\FRM} & {\BCM} & {\BCR} & {\PBC} & {\SPP} & {\FRM} & {\BCM} & {\BCR} \\
         \midrule

  

 GB & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & 0.754{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.668 & 0.617{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.784{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.652 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.667 & 0.619{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} \\ 
  RF & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75 & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & \bfseries 0.8{$^{\scalebox{0.90}{\textbf{\color{blue}*}}}$} & \bfseries 0.662 & 0.75 & \bfseries 0.671 & \bfseries 0.621{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} \\ 
  SR & 0.77 & 0.649 & \bfseries 0.756{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.664 & 0.608 & 0.765 & 0.655 & \bfseries 0.753{$^{\scalebox{0.90}{\textbf{\color{black}*}}}$} & 0.668 & 0.611 \\ 
 
 


  
         \bottomrule
    \end{tabular}
\end{table*}

==> gpformulae2.tex <==
\begin{table*}[h]
    \centering
    %\raggedleft
    \renewcommand{\arraystretch}{1.0}
    \caption{Examples of expressions obtained with SR with different number of dimensions $k$ (no normalization).
    }
    \label{tab:gpformulae}
    \begin{tabular}{p{0.05\textwidth} p{0.001\textwidth} S[table-format=1.3, table-column-width=0.03\textwidth]
        S[table-format=1.3, table-column-width=0.03\textwidth] >{\tiny}l}
         \toprule
 & & \multicolumn{2}{c}{\CI} & \\
         \cmidrule(lr){3-4}
    Dataset & $k$ & {Train} & {Test} & {} \\
         \midrule


\multirow{3}{*}{\SPP} & 3 & 0.715 & 0.647 & $0.176 \log{\left(\left|{x_{1}}\right| \right)} + 0.06 \log{\left(\left|{3.428 x_{27} + 2.681 x_{41}}\right| \right)} - 0.053 \log{\left(\left|{\log{\left(\left|{x_{27}}\right| \right)} + 0.268}\right| \right)} - 1.195$ \\ 
  & 5 & 0.731 & 0.657 & $0.024 \left(x_{17} - 0.389 x_{25}\right)^{2} + 0.175 \log{\left(\left|{x_{1}}\right| \right)} - 0.059 \log{\left(\left|{x_{17}}\right| \right)} + 0.059 \log{\left(\left|{x_{17} + 1.862 x_{25}}\right| \right)} + 0.064 \log{\left(\left|{1.789 x_{27} + 4.592 x_{41}}\right| \right)} - 0.032 \log{\left(\left|{\log{\left(\left|{x_{27}}\right| \right)} + 0.378}\right| \right)} - 0.836$ \\ 

\midrule 
\multirow{3}{*}{\FRM} & 3 & 0.737 & 0.734 & $- 0.745 x_{9}^{2} + 4.104 \log{\left(\left|{x_{1}}\right| \right)} + 46.549$ \\ 
  & 5 & 0.746 & 0.74 & $0.081 x_{1} - 0.431 x_{10} + 0.975 x_{13} - 0.589 x_{9}^{2} - 0.025 \log{\left(\left|{x_{28}}\right| \right)} + 6.771$ \\ 

\midrule 

\multirow{3}{*}{\BCR} & 3 & 0.62 & 0.624 & $- 0.001 x_{1}^{4} + 0.042 x_{3} + 0.051 \log{\left(\left|{x_{6}}\right| \right)}^{2} - 0.051 \log{\left(\left|{x_{6}}\right| \right)} - 0.138 \log{\left(\left|{\log{\left(\left|{x_{1}}\right| \right)}}\right| \right)} - 0.201 - \frac{5.841}{x_{1}^{2} + 1.0}$ \\ 
  & 5 & 0.629 & 0.629 & $- 0.179 x_{27} + 0.041 x_{3} - 1.629 \left(0.328 x_{1} - 1\right)^{2} - 0.015 \log{\left(\left|{x_{36}}\right| \right)} + 0.3 \log{\left(\left|{x_{6} - 3.77}\right| \right)} - 0.065 \log{\left(\left|{\log{\left(\left|{x_{1}}\right| \right)}}\right| \right)} - 0.026 \log{\left(\left|{\log{\left(\left|{x_{6}}\right| \right)}}\right| \right)} + 1.039$ \\ 

 


  
         \bottomrule
    \end{tabular}
\end{table*}
